Least Privilege Access for Persistent Storage Mechanisms in Web Browsers

Web applications often include third-party content and scripts to personalize a user's online experience. These scripts have unrestricted access to a user's private data stored in the browser's persistent storage like cookies, localstorage and IndexedDB, associated with the host page. Various mechanisms have been implemented to restrict access to these storage objects, e.g., content security policy, the HttpOnly attribute with cookies, etc. However, the existing mechanisms provide an all-or-none access and do not work in scenarios where web applications need to allow controlled access to cookies and localstorage objects by third-party scripts. If some of these scripts behave maliciously, they can easily access and modify private user information that are stored in the browser objects. The goal of our work is to design a mechanism to enforce fine-grained control of persistent storage objects. We perform an empirical study of persistent storage access by third-party scripts on Tranco's top 10,000 websites and find that 89.84% of all cookie accesses, 90.98% of all localstorage accesses and 72.49% of IndexedDB accesses are done by third-party scripts. Our approach enforces least privilege access for third-party scripts on these objects to ensure their security by attaching labels to the storage objects that specify which domains are allowed to read from and write to these objects. We implement our approach on the Firefox browser and show that it effectively blocks scripts from other domains, which are not allowed access based on these labels, from accessing the storage objects. We show that our enforcement results in some functionality breakage in websites with the default settings, which can be fixed by correctly labeling the storage objects used by the third-party scripts.

==> discussion.tex <==
\section{Discussion} 

\textbf{Open source anti-tracking lists and classification databases:}
We also ran experiments to obtain the number of cookies, localstorage objects and scripts detected and blocked by well-known tools~\cite{AdGaurd,adservers,AdBlock—97:online,easylist}. 
Tables~\ref{tbl:results6} and~\ref{tbl:results7} show the results of the experiment in the Appendix\ref{sec:appendix}.

For cookies (Table~\ref{tbl:results7}), 50 to 60\% of third-party accesses are identified to be used for advertising and user tracking by these lists~\cite{AdGaurd,adservers,easylist}. Easylist~\cite{easylist} is used in tools like ~\cite{AdBlock—97:online,uBlockOr96:online} to filter adverts from webpages, including unwanted frames, images and objects. AdGuard is also used in tools like \cite{uBlockOr96:online} to filter out advertisements and privacy-invasive content like banners, pop-ups, and trackers. Adserver~\cite{adservers} contains domains that serve ads, tracking scripts and malware.

These percentages indicate that even if anti-tracking tools are used, almost half of them won't be blocked, and their usage will remain unknown. 
In case of localstorage, an average of 33.32\% of the scripts can be blocked using the blocklists as shown in the Table \ref{tbl:results6}. 
%This makes it necessary to have a mechanism to keep track of the requests made by the third-party scripts to the localstorage and cookies so that they can be handled and restricted to do only what they were included for. 
However, these lists do not prevent \emph{specific} websites from accessing \emph{certain} cookies (localstorage objects) while allowing other cookies (localstorage objects) to be accessed.
% \subsection{RQ3: Categorizing the first-party storage items}

We also filtered cookies that are well-known and commonly used in websites by developers for different functionalities, preferences, analytics, and marketing purposes. We used a curated list available from the Open-Cookie-Database~\cite{OpenCook41:online}. As mentioned before, some cookie name-value pairs are also stored as storage objects to avoid the restrictions imposed on cookies. Hence, we repeat the same assessment for localstorage objects. 

% \input{tables/table4} % shows total percentage only 

Tables \ref{tbl:results5} and \ref{tbl:results5b} show which cookies (out of the total 43960) and localstorage objects (out of the total 36989) are classified by the open-cookie-database. In the case of cookies, around 46\% of the cookies shared between third parties are identified based on their usage while in all other categories, the cookies are unique or unidentifiable as per the cookie database. In the case of localstorage items, only 13\% of the total items can be classified using this list as a filter; these storage items are generally stored as cookies.  
    % \item Most of the localstorage items are being used for "marketing".
    % \item Percentage of "functional" storage items is very less.  
%Majority of the cookies involving first-party scripts are "functional". In the case of information flow between third-party scripts, most of the cookies are being used for "analytics".  

% \input{tables/table5}

%\begin{figure} [!tbp]
%\centering
%\begin{tabular}{cccc}
%\includegraphics[width=0.3\textwidth]{images/fp_fp.pdf} &
%\includegraphics[width=0.3\textwidth]{images/fp_tp.pdf} &
%\includegraphics[width=0.3\textwidth]{images/tp_fp.pdf} \\
%\textbf{(a)}  & \textbf{(b)} & \textbf{(c)}  \\[6pt]
%\end{tabular}
%\begin{tabular}{cccc}
%\includegraphics[width=0.3\textwidth]{images/tp_tp_same.pdf} &
%\includegraphics[width=0.3\textwidth]{images/tp_tp_different.pdf} \\
%\textbf{(d)}  & \textbf{(e)}  \\[6pt]
%\end{tabular}
%\caption{ \textbf{(a)} fp\_fp
%\textbf{(b)} fp\_tp
%\textbf{(c)} tp\_fp
%\textbf{(d)} tp\_tp same
%\textbf{(e)} tp\_tp different}
%\label{fig:cookies_func}
%\end{figure}

% \input{tables/table5b}

%\begin{figure} [!tbp]
%\centering
%\begin{tabular}{cccc}
%\includegraphics[width=0.3\textwidth]{images/fp_fp-1.pdf} &
%\includegraphics[width=0.3\textwidth]{images/fp_tp-1.pdf} &
%\includegraphics[width=0.3\textwidth]{images/tp_fp-1.pdf} \\
%\textbf{(a)}  & \textbf{(b)} & \textbf{(c)}  \\[6pt]
%\end{tabular}
%\begin{tabular}{cccc}
%\includegraphics[width=0.3\textwidth]{images/tp_tp_same-1.pdf} &
%\includegraphics[width=0.3\textwidth]{images/tp_tp_different-1.pdf} \\
%\textbf{(d)}  & \textbf{(e)}  \\[6pt]
%\end{tabular}
%\caption{ \textbf{(a)} fp\_fp
%\textbf{(b)} fp\_tp
%\textbf{(c)} tp\_fp
%\textbf{(d)} tp\_tp same
%\textbf{(e)} tp\_tp different}
%\label{fig:storaga_func}
%\end{figure}

As shown above, a significant number of cookies, localstorage objects and scripts cannot be correctly identified using these tools, and hence, cannot be effectively used to control access. 

==> func_breakage.tex <==
\section{Functionality Breakage}

As shown before, certain storage items are used for functional purposes, analytics or marketing, which the user agrees to, to use the site. We manually analyze the effect of our solution for 100 websites where third-party scripts access the host-page cookies (second category described in section \ref{sec:study-methodology}). For this analysis, we manually saved the top 100 websites in the list of websites that contained at least one third-party script accessing  cookies set by the host-page. We then compare the functionality results from the instrumented browser with the unmodified  browser using the comparison tool \emph{meld}~\cite{GNOMEmel24:online}.  
% \newline

% \textbf{Strict Restrictive Least-Privileged Access Browser:} 
By default, in the instrumented browser, the third-party scripts are denied access to the cookies that are created or set by the host servers or the host-page scripts.
We observed that the most affected functionality was the usage of cookie consent management platforms. While the number of advertisements decreased significantly, indicating better user privacy, utility (functionality) was also affected. Some recurring instances of these are listed in Table~\ref{tbl:results9}.
% \newline

We believe that strict measures on the client-side are required for servers to enforce these attributes as part of the Cookie header sent to the client (or to set them programmatically). Once adopted, this approach would provide the host pages fine-grained control over how the third-party scripts access persistent storage objects.

\input{tables/table9}

==> results_old.tex <==
\section{Trend analysis}

We show the results of cookie and localstorage accesses by all scripts on the web page in Table 1. Unsurprisingly, 95\% of the cookies and 91\% of the localstorage objects are being accessed by third-party scripts. Moreover,81.73\% and 84.79\% of all cookies and localstorage accesses (both read and write), respectively, are done by third-party JavaScript.

In case of cookies, out of the 10K websites, 4843 websites had scripts invoking the GetCookie and/or SetCookie APIs. More detailed analysis indicated the following:

\begin{itemize}
    \item In about 20.14\% accesses, cookies were set by first-party scripts and accessed by third-party scripts. 
    \item 0.54\% of the cookies set by third-party scripts are used by first-party scripts. 
    \item 4.87\% of the cookies are not accessed by third-party scripts. 
    \item 74.3\% of the cookies are shared between different third-party scripts. 
\end{itemize}




\begin{table}[htbp]
\caption{Tranco Top 10K first-party storage accesses}
\label{tbl:results1}
\begin{center}
\resizebox{0.5\textwidth}{!} 
{ 

\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Access API} & \textbf{First-party access} & \textbf{Third-party access} & \textbf{\% third-party access} \\ \hline
\textbf{GetCookie}  & 361234                      & 1420638                     & 79.73                          \\ \hline
\textbf{SetCookie}  & 21269                       & 290010                      & 93.17                          \\ \hline
\textbf{GetItem}    & 36238                       & 201233                      & 84.74                          \\ \hline
\textbf{SetItem}    & 12253                       & 69198                       & 84.95                          \\ \hline
\end{tabular}
}
\end{center}
\end{table}

In case of localstorage,the logs captured requests from 3717 websites out of the 10K websites. Detailed analysis indicated these observations:
\begin{itemize}
   \item Around 76\% of localstorage items set by first-party scripts are accessed by third-party scripts.  
    \item 0.14\% of the localStorage items set by third-party scripts are used by first-party scripts. 
    \item \~9.2\% of the localstorage items are not shared with third-party scripts. 
    \item 14.66\% of the localstorage items are shared between third-party scripts. 
\end{itemize}

\paragraph{\textbf{Possible violations:}} We also found a few instances where third-party scripts \emph{not} belonging to the domain of a consent management provider modified consent-related objects. In particular,  localstorage objects with keys \textsf{cookieConsent*} in \textsf{us.diablo3.blizzard.com} and \textsf{blizzcon.com} are modified by scripts from \textsf{connect.facebook.net}. 
% Moreover they don't mention these localstorage items in the privacy policy. 
Another example of such an access is the item  \textsf{osano\_consentmanager\_*} used by \textsf{grammy.com} but modified by a script from \textsf{securepubads.g.doubleclick.net}.

\section{Towards Least-Privilege Access}
\label{rq-lpa}
To prevent unauthorized access for persistent storage objects by third-party scripts, we propose a least-privilege access solution using the notion of labels. We attach fine-grained labels or taints (similar to decentralized labels~\cite{dlm}) with cookies and web-storage objects when they are stored in the browser; these labels are sets of domains --- $(\{r_1, r_2\}, \{w_1, w_2\})$ --- that have access to read from/write to the object. The first set specifies the readers while the second set specifies the writers for a particular object. 
Every access to these objects is then subject to access checks comparing the domain of the script accessing the object and the domains contained in the read-set or the write-set. Note that the original store in the browser that maps domain names to cookies and localstorage objects is unchanged, making it easier to retrieve the owners of these objects. 

To populate these labels for cookies in the browser, we propose that the server sends additional attributes along with the cookie specifying the domains that are allowed access to read/modify the cookie. A cookie created on the client-side by any of the scripts is added to the cookie store of the host page with the script's domain having read-write access to the cookie. For sharing these cookies with other third-party scripts, the script needs to set the proper attributes for that cookie failing which the cookie will only be accessible by the host page and the creator-script's domain. 

In the case of localstorage, we allow scripts (from same domains) creating the object to specify the readers and writers of a particular object by exposing additional APIs --- \textsf{setReaders (key, list\_of\_domains)} and \textsf{setWriters (key, list\_of\_domains)}. Without these set, the localstorge object is only accessible by the script's domain other than the host page. 



==> tables/table00.tex <==
\begin{table*}[!tbp]
\caption{Tranco Top 10K storage accesses}
\label{tbl:results00}
\centering
\begin{adjustbox}{max width=\textwidth}

\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Type of access} & \textbf{Total first-party access} & \textbf{Total third-party access} & \textbf{\% of third-party access} \\ \hline
\textbf{GetItem}        & 36238                             & 201233                            & 84.74                             \\ \hline
\textbf{SetItem}        & 12253                             & 69198                             & 84.95                             \\ \hline
\textbf{Total}          & 48491                             & 270434                            & 84.79                             \\ \hline
\end{tabular}

\end{adjustbox}
\end{table*}

==> tables/table1.tex <==
\begin{table*}[!tbp]
\centering
% \begin{adjustbox}{width=\columnwidth}
\begin{tabular}{|c|P{1.2in}|P{0.5in}P{0.5in}|cccc|}
\hline
\multirow{2}{*}{\textbf{1st Access}}                             & \textbf{Subsequent Access} & \multicolumn{2}{c|}{\textbf{First-party}}        & \multicolumn{4}{c|}{\textbf{Third-party}}                                                                                                                                               \\ \cline{2-8}
                   & \textbf{Type of access}         & \multicolumn{1}{P{0.5in}|}{\textbf{Get}} & \textbf{Set} & \multicolumn{2}{P{1.4in}|}{\textbf{Get}}                                                          & \multicolumn{2}{P{1.4in}|}{\textbf{Set}}                                                                \\ \hline
\multirow{3}{*}{\textbf{First-party}} & \textbf{\#Storage elements}               & \multicolumn{1}{c|}{2757}         & 647                               & \multicolumn{2}{c|}{861}                                                                   & \multicolumn{2}{c|}{179}                                                                   \\ \cline{2-8} 
                                      & \textbf{\#Scripts which accessed}         & \multicolumn{1}{c|}{27505}        & 3704                              & \multicolumn{2}{c|}{29140}                                                                 & \multicolumn{2}{c|}{2060}                                                                  \\ \cline{2-8} 
                                      & \textbf{\#Websites}                       & \multicolumn{1}{c|}{868}          & 405                               & \multicolumn{2}{c|}{326}                                                                   & \multicolumn{2}{c|}{127}                                                                   \\ \hline
\multirow{4}{*}{\textbf{Third-party}}                                      &                                           & \multicolumn{1}{c|}{}             &              & \multicolumn{1}{P{0.7in}|}{\textbf{Same Domain}} & \multicolumn{1}{P{0.7in}|}{\textbf{Different Domain}} & \multicolumn{1}{P{0.7in}|}{\textbf{Same domain}} & \multicolumn{1}{P{0.7in}|}{\textbf{Different Domain}} \\ \cline{2-8}
     & \textbf{\#Storage elements}               & \multicolumn{1}{c|}{518}          & 54                                & \multicolumn{1}{c|}{16722}                & \multicolumn{1}{c|}{9281}                      & \multicolumn{1}{c|}{3889}                 & 1541                                           \\ \cline{2-8} 
                                      & \textbf{\#Scripts which accessed}         & \multicolumn{1}{c|}{16433}        & 450                               & \multicolumn{1}{c|}{79512}                & \multicolumn{1}{c|}{118081}                    & \multicolumn{1}{c|}{16772}                & 13170                                          \\ \cline{2-8} 
                                      & \textbf{\#Websites}                       & \multicolumn{1}{c|}{177}          & 47                                & \multicolumn{1}{c|}{2657}                 & \multicolumn{1}{c|}{1452}                      & \multicolumn{1}{c|}{1691}                 & 653                                            \\ \hline
\end{tabular}
% \end{adjustbox}
\caption{Localstorage object accesses}
\label{tbl:results}
\end{table*}

==> tables/table11.tex <==
\begin{table}[h!]
\caption{Tranco Top 10K first-party storage accesses}
\label{tbl:results1}
\begin{center}
\resizebox{0.4\textwidth}{!} 
{ 

\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Access API} & \textbf{First-party access} & \textbf{Third-party access} & \textbf{\% third-party access} \\ \hline
\textbf{GetCookie}  & 361234                      & 1420638                     & 79.73                          \\ \hline
\textbf{SetCookie}  & 21269                       & 290010                      & 93.17                          \\ \hline
\textbf{GetItem}    & 36238                       & 201233                      & 84.74                          \\ \hline
\textbf{SetItem}    & 12253                       & 69198                       & 84.95                          \\ \hline
\end{tabular}
}
\end{center}
\end{table}


==> tables/table2.tex <==
\begin{table}[!tbp]
\centering
% \begin{table}[]
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{|c|P{1.2in}|P{0.5in}P{0.5in}|cccc|}
\hline
\multirow{2}{*}{\textbf{1st Access}}                             & \textbf{Subsequent Access} & \multicolumn{2}{c|}{\textbf{First-party}}        & \multicolumn{4}{c|}{\textbf{Third-party}}                                                                                                                                               \\ \cline{2-8}
                   & \textbf{Type of access}         & \multicolumn{1}{P{0.5in}|}{\textbf{Get}} & \textbf{Set} & \multicolumn{2}{P{1.4in}|}{\textbf{Get}}                                                          & \multicolumn{2}{P{1.4in}|}{\textbf{Set}}                                                          \\ \hline
\multirow{3}{*}{\textbf{First-party}} & \textbf{\#Cookies elements}               & \multicolumn{1}{c|}{343}          & 1797         & \multicolumn{2}{c|}{641}                                                                   & \multicolumn{2}{c|}{2989}                                                                  \\ \cline{2-8} 
                                      & \textbf{\#Scripts which accessed}         & \multicolumn{1}{c|}{18475}        & 18840        & \multicolumn{2}{c|}{273209}                                                                & \multicolumn{2}{c|}{71979}                                                                 \\ \cline{2-8} 
                                      & \textbf{\#Websites}                       & \multicolumn{1}{c|}{332}          & 675          & \multicolumn{2}{c|}{628}                                                                   & \multicolumn{2}{c|}{195}                                                                   \\ \hline
\multirow{4}{*}{\textbf{Third-party}}                                      &                                           & \multicolumn{1}{c|}{}             &              & \multicolumn{1}{P{0.7in}|}{\textbf{Same Domain}} & \multicolumn{1}{P{0.7in}|}{\textbf{Different Domain}} & \multicolumn{1}{P{0.7in}|}{\textbf{Same domain}} & \multicolumn{1}{P{0.7in}|}{\textbf{Different Domain}} \\ \cline{2-8}
       & \textbf{\#Cookies elements}               & \multicolumn{1}{c|}{499}          & 210          & \multicolumn{1}{c|}{4747}                 & \multicolumn{1}{c|}{2824}                      & \multicolumn{1}{c|}{29910}                & 2752                                           \\ \cline{2-8} 
                                      & \textbf{\#Scripts which accessed}         & \multicolumn{1}{c|}{263974}       & 83736        & \multicolumn{1}{c|}{975621}               & \multicolumn{1}{c|}{888077}                    & \multicolumn{1}{c|}{735027}               & 464016                                         \\ \cline{2-8} 
                                      & \textbf{\#Websites}                       & \multicolumn{1}{c|}{493}          & 183          & \multicolumn{1}{c|}{3982}                 & \multicolumn{1}{c|}{2576}                      & \multicolumn{1}{c|}{3802}                 & 1901                                           \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Tranco top 10K cookie accesses}
\label{tbl:results2}
\end{table}

==> tables/table22.tex <==
\begin{table}[htbp]
\caption{Categories of third-party script accesses}
\label{tbl:results2}
\begin{center}
\begin{tabular}{|l|l|l|}
\hline
\textbf{Website category}   & \textbf{Most tracked websites} & \textbf{Alexa top 1.6K}                                                     \\ \hline
\textbf{Third-party access} & \textbf{136 unique out of 403} & \textbf{\begin{tabular}[c]{@{}l@{}}1026 unique\\ out  of 5717\end{tabular}} \\ \hline
\textbf{AdGaurd}            & 51                             & 196                                                                         \\ \hline
\textbf{EasyList}           & 15                             & 32                                                                          \\ \hline
\textbf{Facebook services}  & 1                              & 4                                                                           \\ \hline
\end{tabular}
\end{center}
\end{table}

==> tables/table3.tex <==
\begin{table}[!tbp]
\centering
\caption{Categories of third-party script accesses}
\label{tbl:results3}
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|rrr|rrr|}
\hline
\textbf{Website category}   & \multicolumn{3}{c|}{\textbf{Most tracked websites}}                                                                       & \multicolumn{3}{c|}{\textbf{Alexa top 1.6K}}                                                                              \\ \hline
\textbf{}                   & \multicolumn{1}{l|}{\textbf{Get cookie}} & \multicolumn{1}{l|}{\textbf{Set Cookie}} & \multicolumn{1}{l|}{\textbf{Total}} & \multicolumn{1}{l|}{\textbf{Get cookie}} & \multicolumn{1}{l|}{\textbf{Set Cookie}} & \multicolumn{1}{l|}{\textbf{Total}} \\ \hline
\textbf{Third-party access} & \multicolumn{1}{r|}{129}                 & \multicolumn{1}{r|}{89}                  & 218                                 & \multicolumn{1}{r|}{1956}                & \multicolumn{1}{r|}{3327}                & 5283                                \\ \hline
\textbf{AdGaurd}            & \multicolumn{1}{r|}{47}                  & \multicolumn{1}{r|}{35}                  & 82                                  & \multicolumn{1}{r|}{406}                 & \multicolumn{1}{r|}{320}                 & 726                                 \\ \hline
\textbf{EasyList}           & \multicolumn{1}{r|}{14}                  & \multicolumn{1}{r|}{10}                  & 24                                  & \multicolumn{1}{r|}{79}                  & \multicolumn{1}{r|}{41}                  & 120                                 \\ \hline
\textbf{Facebook}           & \multicolumn{1}{r|}{1}                   & \multicolumn{1}{r|}{1}                   & 2                                   & \multicolumn{1}{r|}{4}                   & \multicolumn{1}{r|}{2}                   & 6                                   \\ \hline
\textbf{Coin miners}        & \multicolumn{1}{r|}{0}                   & \multicolumn{1}{r|}{0}                   & 0                                   & \multicolumn{1}{r|}{2}                   & \multicolumn{1}{r|}{1}                   & 3                                   \\ \hline
\textbf{AdServers}          & \multicolumn{1}{r|}{44}                  & \multicolumn{1}{r|}{38}                  & 82                                  & \multicolumn{1}{r|}{280}                 & \multicolumn{1}{r|}{207}                 & 487                                 \\ \hline
\end{tabular}
}
\end{table}



==> tables/table4.tex <==
\begin{table*}[!tbp]
\caption{Identifiable cookies and localstorage items}
\label{tbl:results4}
\centering
\begin{adjustbox}{max width=\textwidth}
\subfloat[Cookies]{
\begin{tabular}{|l|l|l|}
\hline
                                   & \textbf{Total}     & \textbf{Unique} \\ \hline
\textbf{First-party - First-Party} & 212/2140=10\%      & 62/1161=5.3\%   \\ \hline
\textbf{First-party - Third-Party} & 154/878=17.5\%     & 42/411=10.2\%   \\ \hline
\textbf{Third-party - First-Party} & 198/709=28\%       & 34/341=10\%     \\ \hline
\textbf{Same Third-Parties}        & 11958/34657=34.5\% & 150/10179=1.4\% \\ \hline
\textbf{Different Third-Parties}   & 2584/5576=46.3\%   & 81/1485=5.4\%   \\ \hline
\end{tabular}
}

\quad
\subfloat[LocalStorage Items]{

\begin{tabular}{|l|l|l|}
\hline
                                   & \textbf{Total}  & \textbf{Unique} \\ \hline
\textbf{First-party - First-Party} & 68/3404=1\%     & 24/2014=1.2\%   \\ \hline
\textbf{First-party - Third-Party} & 13/1040=1\%     & 10/659=1.5\%    \\ \hline
\textbf{Third-party - First-Party} & 20/572=3.4\%    & 9/343=2.6\%     \\ \hline
\textbf{Same Third-Parties}        & 636/20611=3\%   & 34/6772=0.5\%   \\ \hline
\textbf{Different Third-Parties}   & 409/11362=3.6\% & 23/3470=0.6\%   \\ \hline
\end{tabular}
}
\end{adjustbox}
\end{table*}

==> tables/table5.tex <==
\begin{table*}[!tbp]
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Cookies} & \textbf{Accessed by} & \textbf{Total}            & \textbf{Functional} & \textbf{Analytics} & \textbf{Marketing}  \\ \hline
\multirow{2}{*}{\textbf{First-party}} & \textbf{First-Party} & 2140 & 79 (3.6\%)       & 70 (3.2\%)      & 63 (2.9\%)    \\ \cline{2-6}
 & \textbf{Third-Party} & 878 & 108 (12.3\%)      & 21 (2.4\%)       & 25 (2.8\%)          \\ \hline
\multirow{3}{*}{\textbf{Third-party}} & \textbf{First-Party} & 709 & 107 (15\%)        & 44 (6.2\%)       & 47 (6.6\%)         \\ \cline{2-6}
&\textbf{Same Third-Party}        & 34657 & 2035 (5.8\%)    & 6587 (19\%)    & 3336 (9\%)         \\ \cline{2-6}
&\textbf{Different Third-Party}   & 5576 & 447 (8\%)        & 1659 (29.7\%)   & 478 (8.5\%)    \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Cookies accessed by JavaScript classified in open-cookie-database}
\label{tbl:results5}
\end{table*}

==> tables/table5b.tex <==
\begin{table*}[!tbp]
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Localstorage} & \textbf{Accessed by} & \textbf{Total}            & \textbf{Functional} & \textbf{Analytics} & \textbf{Marketing}  \\ \hline
\multirow{2}{*}{\textbf{First-party}} & \textbf{First-Party} & 3404 & 7 (0.2\%)        & 18 (0.5\%)      & 43 (1.2\%)           \\ \cline{2-6}
 & \textbf{Third-Party} & 1040 & 2 (0.2\%)        & 2 (0.2\%)       & 9 (0.8\%)              \\ \hline
\multirow{3}{*}{\textbf{Third-party}} & \textbf{First-Party} & 572 & 0\%                 & 3 (0.5\%)        & 17 (2.9\%)       \\ \cline{2-6}
& \textbf{Same Third-Party} & 20611        & 61 (0.3\%)      & 186 (0.9\%)    & 389 (1.8\%)            \\ \cline{2-6}
& \textbf{Different Third-Party} & 11362  & 6 (0.05\%)      & 51 (0.45\%)    & 352 (3.1\%)        \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Localstorage accessed by JavaScript classified in open-cookie-database}
\label{tbl:results5b}
\end{table*}

==> tables/table6.tex <==
\begin{table}[htbp]
\centering
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{|c|c|c|c|c|}
\hline
                                   & \textbf{Total} & \textbf{AdGaurd}~\cite{AdGaurd}    & \textbf{EasyList}~\cite{easylist}  & \textbf{AdServers}~\cite{adservers} \\ \hline
\textbf{First-party - Third-Party} & 22965 & 10651 (46\%)    & 1806 (7.9\%)   & 4832 (21\%)    \\ \hline
\textbf{Third-party - First-Party} & 9831 & 3031 (30.8\%)    & 1577 (16\%)     & 4722 (48\%)     \\ \hline
\textbf{Same Third-Parties}        & 96284 & 40040 (41.5\%)  & 6607 (6.8\%)   & 39608 (41.1\%) \\ \hline
\textbf{Different Third-Parties}   & 75174 & 26501 (35.25\%) & 10792 (14.3\%) & 42472 (56.5\%) \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Number of localstorage accesses tagged by existing tools}
\label{tbl:results6}
\end{table}

==> tables/table7.tex <==
\begin{table}[htbp]
\centering
\begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{|c|c|c|c|c|}
\hline
                                   & \textbf{Total} & \textbf{AdGuard}~\cite{AdGaurd}     & \textbf{EasyList}~\cite{easylist}   & \textbf{AdServers}~\cite{adservers}   \\ \hline
\textbf{First-party - Third-Party} & 250283 & 124700 (49.8\%) & 13022 (5\%)    & 152403 (60\%)   \\ \hline
\textbf{Third-party - First-Party} & 285102 & 144893 (51\%)   & 15206 (5\%)    & 152403 (61\%0   \\ \hline
\textbf{Same Third-Parties}        & 615902 & 303477 (49.2\%) & 31309 (5\%)    & 368361 (59.8\%) \\ \hline
\textbf{Different Third-Parties}   & 1289485 & 544886 (42\%)  & 71332 (5.5\%) & 853249 (66\%)  \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Number of cookie accesses tagged by different tools}
\label{tbl:results7}
\end{table}

==> tables/table8.tex <==
\begin{table}[htbp]
\centering
% \begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{|p{2.5cm}|p{5.5cm}|}
% \begin{tabular}{|l|l|}
\hline
\textbf{Cookie name}                & \textbf{Website name}                                                                                                                                                                                                                 \\ \hline
notion\_check \_cookie\_consent      & notion.so                                                                                                                                                                                                                             \\ \hline
OptanonConsent                      & www.eyeota.com, elisaviihde.fi, www.razer.com, www.exoclick.com, www.instructure.com,  www.vonage.com,  www.bodybuilding.com, www.moonpay.com, www.ledger.com,  www.narrative.io, 74 more \\ \hline
gdpr\_consent                       & www.wufoo.com                                                                                                                                                                                                                         \\ \hline
\_pbjs\_userid \_consent\_data       & www.drugs.com, www.infoseek.co.jp, drudgereport.com , www.businessinsider.in,  www.timesofisrael.com , www.cityam.com, www.rogerebert.com, www.aip.org                                      \\ \hline
osano\_consent manager\_uuid         & www.ada.cx, www.osano.com , www.bitcoin.com, buffalonews.com, shopping.buffalonews.com,  www.linuxfoundation.org, lolesports.com,  www.geotab.com, omaha.com                                \\ \hline
euconsent-bypass                    & Web.de, www.gmx.net                                                                                                                                                                                                                   \\ \hline
gaia\_cookie\_ consent-version       & www.anu.edu.au                                                                                                                                                                                                                        \\ \hline
uncode\_privacy {[}consent\_types{]} & Lifeomic.com                                                                                                                                                                                                                          \\ \hline
cookiebot-consent--necessary        & www.avl.com, www.aalto.fi, oscars.org, fsc.org,                                                                                                                                                                                       \\ \hline
indg-cookieConsent                  & www.bloombergindustry.com                                                                                                                                                                                                             \\ \hline
lolg\_euconsent                     & www.leagueofgraphs.com                                                                                                                                                                                                                \\ \hline
cookie-banner-consent-accepted      & www.techtudo.com.br                                                                                                                                                                                                                   \\ \hline
\end{tabular}
% \end{adjustbox}
\caption{Consent related cookies}
\label{tbl:results8}
\end{table}
